$(g-2)_{e,\mu}$ anomalies and decays $h\to e_a e_b$, $Z\to e_ae_b$, and $e_b\to e_a \gamma$ in a two Higgs doublet model with inverse seesaw neutrinos

The lepton flavor violating decays $h\to e_b^\pm e_a^\mp $, $Z\to e_b^\pm e_a^\mp$, and $e_b\to e_a \gamma$ will be discussed in the framework of the Two Higgs doublet model with presence of new inverse seesaw neutrinos and a singly charged Higgs boson that accommodate both $1\sigma$ experimental data of $(g-2)$ anomalies of the muon and electron. Numerical results indicate that there exist regions of the parameter space supporting all experimental data of $(g-2)_{e,\mu}$ as well as the promising LFV signals corresponding to the future experimental sensitivities.

==> biblio_RxiISS.tex <==
\bibitem{Jurciukonis:2021izn}
D.~Jur\v{c}iukonis and L.~Lavoura,
%``Two-body lepton-flavour-violating decays in a 2HDM with soft family-lepton-number breaking,''
JHEP \textbf{03} (2022), 106
%doi:10.1007/JHEP03(2022)106
[arXiv:2107.14207 [hep-ph]].




\bibitem{Parker:2018vye}
R.~H.~Parker, C.~Yu, W.~Zhong, B.~Estey and H.~M\"uller,
%``Measurement of the fine-structure constant as a test of the Standard Model,''
Science \textbf{360} (2018), 191
%doi:10.1126/science.aap7706
[arXiv:1812.04130 [physics.atom-ph]].

\bibitem{Fan:2022eto}
X.~Fan, T.~G.~Myers, B.~A.~D.~Sukra and G.~Gabrielse,
%``Measurement of the Electron Magnetic Moment,''
Phys. Rev. Lett. \textbf{130} (2023) no.7, 071801
%doi:10.1103/PhysRevLett.130.071801
[arXiv:2209.13084 [physics.atom-ph]].

\bibitem{Muong-2:2023cdq}
D.~P.~Aguillard \textit{et al.} [Muon g-2],
%``Measurement of the Positive Muon Anomalous Magnetic Moment to 0.20~ppm,''
Phys. Rev. Lett. \textbf{131} (2023) no.16, 161802
%doi:10.1103/PhysRevLett.131.161802
[arXiv:2308.06230 [hep-ex]].

\bibitem{Mondal:2021vou}
T.~Mondal and H.~Okada,
%``Inverse seesaw and (g \ensuremath{-} 2) anomalies in B \ensuremath{-} L extended two Higgs doublet model,''
Nucl. Phys. B \textbf{976}, 115716 (2022)
%doi:10.1016/j.nuclphysb.2022.115716
[arXiv:2103.13149 [hep-ph]].



\bibitem{Hue:2023rks}
L.~T.~Hue, H.~N.~Long, V.~H.~Binh, H.~L.~T.~Mai and T.~P.~Nguyen,
%``One-loop contributions to decays eb \textrightarrow{} ea\ensuremath{\gamma} and (g\ensuremath{-}2)ea anomalies, and Ward identity,''
Nucl. Phys. B \textbf{992}, 116244 (2023)
%doi:10.1016/j.nuclphysb.2023.116244
[arXiv:2301.05407 [hep-ph]].




\bibitem{Crivellin:2018qmi}
A.~Crivellin, M.~Hoferichter and P.~Schmidt-Wellenburg,
%``Combined explanations of $(g-2)_{\mu,e}$ and implications for a large muon EDM,''
Phys. Rev. D \textbf{98}, no.11, 113002 (2018)
%doi:10.1103/PhysRevD.98.113002
[arXiv:1807.11484 [hep-ph]].

\bibitem{Hong:2022xjg}
T.~T.~Hong, N.~H.~T.~Nha, T.~P.~Nguyen, L.~T.~T.~Phuong and L.~T.~Hue,
%``Decays h \textrightarrow{} eaeb, eb \textrightarrow{} ea\ensuremath{\gamma}, and (g \ensuremath{-} 2)e,\ensuremath{\mu} in a 3-3-1 model with inverse seesaw neutrinos,''
PTEP \textbf{2022} (2022) no.9, 093B05
%doi:10.1093/ptep/ptac109
[arXiv:2206.08028 [hep-ph]].

\bibitem{CortesMaldonado:2011uh}
I.~Cortes Maldonado, A.~Moyotl and G.~Tavares-Velasco,
%``Lepton flavor violating decay $Z\to \ell^\pm_i \ell^\pm_j$ in the 331 model,''
Int. J. Mod. Phys. A \textbf{26} (2011), 4171-4185
%doi:10.1142/S0217751X11054474
[arXiv:1109.0661 [hep-ph]].


\bibitem{Dermisek:2020cod}
R.~Dermisek, K.~Hermanek, N.~McGinnis and N.~McGinnis,
%``Highly Enhanced Contributions of Heavy Higgs Bosons and New Leptons to Muon $g$\ensuremath{-}2 and Prospects at Future Colliders,''
Phys. Rev. Lett. \textbf{126} (2021) no.19, 191801
%doi:10.1103/PhysRevLett.126.191801
[arXiv:2011.11812 [hep-ph]].

\bibitem{Dermisek:2021ajd}
R.~Dermisek, K.~Hermanek and N.~McGinnis,
%``Muon g-2 in two-Higgs-doublet models with vectorlike leptons,''
Phys. Rev. D \textbf{104} (2021) no.5, 055033
%doi:10.1103/PhysRevD.104.055033
[arXiv:2103.05645 [hep-ph]].

\bibitem{Dermisek:2022aec}
R.~Dermisek, K.~Hermanek, N.~McGinnis and S.~Yoon,
%``Ellipse of Muon Dipole Moments,''
Phys. Rev. Lett. \textbf{129} (2022) no.22, 221801
%doi:10.1103/PhysRevLett.129.221801
[arXiv:2205.14243 [hep-ph]].

\bibitem{DeJesus:2020yqx}
A.~S.~De Jesus, S.~Kovalenko, F.~S.~Queiroz, C.~Siqueira and K.~Sinha,
%``Vectorlike leptons and inert scalar triplet: Lepton flavor violation, $g-2$, and collider searches,''
Phys. Rev. D \textbf{102} (2020) no.3, 035004
%doi:10.1103/PhysRevD.102.035004
[arXiv:2004.01200 [hep-ph]].

\bibitem{Cogollo:2020nrc}
D.~Cogollo, Y.~M.~Oviedo-Torres and Y.~S.~Villamizar,
%``Are 3-4-1 models able to explain the upcoming results of the muon anomalous magnetic moment?,''
Int. J. Mod. Phys. A \textbf{35} (2020) no.23, 2050126
%doi:10.1142/S0217751X20501262
[arXiv:2004.14792 [hep-ph]].

\bibitem{Dermisek:2023tgq}
R.~Dermisek, K.~Hermanek, N.~McGinnis and S.~Yoon,
%``Predictions for muon electric and magnetic dipole moments from h\textrightarrow{}\ensuremath{\mu}+\ensuremath{\mu}- in two-Higgs-doublet models with new leptons,''
Phys. Rev. D \textbf{108} (2023) no.5, 055019
%doi:10.1103/PhysRevD.108.055019
[arXiv:2306.13212 [hep-ph]].

\bibitem{deJesus:2023som}
\'A.~S.~de Jesus, F.~S.~Queiroz, J.~W.~F.~Valle and Y.~Villamizar,
%``Vector-Like Fermions and Inert Scalar Solutions to the Muon g-2 Anomaly and collider probes at the HL-LHC and FCC-hh,''
[arXiv:2312.03851 [hep-ph]].

\bibitem{Arganda:2014dta}
E.~Arganda, M.~J.~Herrero, X.~Marcano and C.~Weiland,
%``Imprints of massive inverse seesaw model neutrinos in lepton flavor violating Higgs boson decays,''
Phys. Rev. D \textbf{91} (2015) no.1, 015001
%doi:10.1103/PhysRevD.91.015001
[arXiv:1405.4300 [hep-ph]].

\bibitem{Herrero:2017myd}
M.~J.~Herrero, E.~Arganda, X.~Marcano, R.~Morales and A.~Szynkman,
%``Higgs effective $\boldsymbol{H\ell_i\ell_j}$ vertex from heavy $\boldsymbol{\nu_R}$ and applications to LFV phenomenology,''
PoS \textbf{EPS-HEP2017} (2017), 114
%doi:10.22323/1.314.0114
[arXiv:1710.02510 [hep-ph]]

\bibitem{Arganda:2016zvc}
E.~Arganda, M.~J.~Herrero, X.~Marcano, R.~Morales and A.~Szynkman,
%``Effective lepton flavor violating H\ensuremath{\ell}i\ensuremath{\ell}j vertex from right-handed neutrinos within the mass insertion approximation,''
Phys. Rev. D \textbf{95} (2017) no.9, 095029
%doi:10.1103/PhysRevD.95.095029
[arXiv:1612.09290 [hep-ph]].

\bibitem{Korner:1992an}
J.~G.~Korner, A.~Pilaftsis and K.~Schilcher,
%``Leptonic flavor changing Z0 decays in SU(2) x U(1) theories with right-handed neutrinos,''
Phys. Lett. B \textbf{300} (1993), 381-386
%doi:10.1016/0370-2693(93)91350-V
[arXiv:hep-ph/9301290 [hep-ph]].


\bibitem{DeRomeri:2016gum}
V.~De Romeri, M.~J.~Herrero, X.~Marcano and F.~Scarcella,
%``Lepton flavor violating Z decays: A promising window to low scale seesaw neutrinos,''
Phys. Rev. D \textbf{95} (2017) no.7, 075028
%doi:10.1103/PhysRevD.95.075028
[arXiv:1607.05257 [hep-ph]].

\bibitem{Hernandez-Tome:2019lkb}
G.~Hern\'andez-Tom\'e, J.~I.~Illana, M.~Masip, G.~L\'opez Castro and P.~Roig,
%``Effects of heavy Majorana neutrinos on lepton flavor violating processes,''
Phys. Rev. D \textbf{101} (2020) no.7, 075020
%doi:10.1103/PhysRevD.101.075020
[arXiv:1912.13327 [hep-ph]].

\bibitem{Abada:2022asx}
A.~Abada, J.~Kriewald, E.~Pinsard, S.~Rosauro-Alcaraz and A.~M.~Teixeira,
%``LFV Higgs and Z-boson decays: leptonic CPV phases and CP asymmetries,''
Eur. Phys. J. C \textbf{83} (2023) no.6, 494
%doi:10.1140/epjc/s10052-023-11585-w
[arXiv:2207.10109 [hep-ph]].


\bibitem{ATLAS:2020tre}
G.~Aad \textit{et al.} [ATLAS],
%``Search for lepton-flavour violation in high-mass dilepton final states using 139 fb$^{−1}$ of pp collisions at $ \sqrt{s} $ = 13 TeV with the ATLAS detector,''
JHEP \textbf{23} (2020), 082
%doi:10.1007/JHEP10(2023)082
[arXiv:2307.08567 [hep-ex]].


\bibitem{Aoyama:2020ynm}
T.~Aoyama, N.~Asmussen, M.~Benayoun, J.~Bijnens, T.~Blum, M.~Bruno, I.~Caprini, C.~M.~Carloni Calame, M.~C\`e and G.~Colangelo, \textit{et al.}
%``The anomalous magnetic moment of the muon in the Standard Model,''
Phys. Rept. \textbf{887}, 1-166 (2020)
%doi:10.1016/j.physrep.2020.07.006
[arXiv:2006.04822 [hep-ph]].


%%%%%(g-2)mu
\bibitem{Davier:2010nc}
M.~Davier, A.~Hoecker, B.~Malaescu and Z.~Zhang,
%``Reevaluation of the Hadronic Contributions to the Muon g-2 and to alpha(MZ),''
Eur. Phys. J. C \textbf{71}, 1515 (2011)
[erratum: Eur. Phys. J. C \textbf{72}, 1874 (2012)]
%doi:10.1140/epjc/s10052-012-1874-8
[arXiv:1010.4180 [hep-ph]].

\bibitem{Aoyama:2012wk}
T.~Aoyama, M.~Hayakawa, T.~Kinoshita and M.~Nio,
%``Complete Tenth-Order QED Contribution to the Muon g-2,''
Phys. Rev. Lett. \textbf{109}, 111808 (2012)
%doi:10.1103/PhysRevLett.109.111808
[arXiv:1205.5370 [hep-ph]].

\bibitem{Aoyama:2019ryr}
T.~Aoyama, T.~Kinoshita and M.~Nio,
%``Theory of the Anomalous Magnetic Moment of the Electron,''
Atoms \textbf{7}, no.1, 28 (2019)
%doi:10.3390/atoms7010028

\bibitem{Czarnecki:2002nt}
A.~Czarnecki, W.~J.~Marciano and A.~Vainshtein,
%``Refinements in electroweak contributions to the muon anomalous magnetic moment,''
Phys. Rev. D \textbf{67}, 073006 (2003)
[erratum: Phys. Rev. D \textbf{73}, 119901 (2006)]
%doi:10.1103/PhysRevD.67.073006
[arXiv:hep-ph/0212229 [hep-ph]].

\bibitem{Gnendiger:2013pva}
C.~Gnendiger, D.~St\"ockinger and H.~St\"ockinger-Kim,
%``The electroweak contributions to $(g-2)_\mu$ after the Higgs boson mass measurement,''
Phys. Rev. D \textbf{88}, 053005 (2013)
%doi:10.1103/PhysRevD.88.053005
[arXiv:1306.5546 [hep-ph]].

\bibitem{Danilkin:2016hnh}
I.~Danilkin and M.~Vanderhaeghen,
%``Light-by-light scattering sum rules in light of new data,''
Phys. Rev. D \textbf{95}, no.1, 014019 (2017)
%doi:10.1103/PhysRevD.95.014019
[arXiv:1611.04646 [hep-ph]].

\bibitem{Davier:2017zfy}
M.~Davier, A.~Hoecker, B.~Malaescu and Z.~Zhang,
%``Reevaluation of the hadronic vacuum polarisation contributions to the Standard Model predictions of the muon $g-2$ and ${\alpha (m_Z^2)}$ using newest hadronic cross-section data,''
Eur. Phys. J. C \textbf{77}, no.12, 827 (2017)
%doi:10.1140/epjc/s10052-017-5161-6
[arXiv:1706.09436 [hep-ph]].

\bibitem{Keshavarzi:2018mgv}
A.~Keshavarzi, D.~Nomura and T.~Teubner,
%``Muon $g-2$ and $\alpha(M_Z^2)$: a new data-based analysis,''
Phys. Rev. D \textbf{97}, no.11, 114025 (2018)
%doi:10.1103/PhysRevD.97.114025
[arXiv:1802.02995 [hep-ph]].

\bibitem{Colangelo:2018mtw}
G.~Colangelo, M.~Hoferichter and P.~Stoffer,
%``Two-pion contribution to hadronic vacuum polarization,''
JHEP \textbf{02}, 006 (2019)
%doi:10.1007/JHEP02(2019)006
[arXiv:1810.00007 [hep-ph]].

\bibitem{Hoferichter:2019mqg}
M.~Hoferichter, B.~L.~Hoid and B.~Kubis,
%``Three-pion contribution to hadronic vacuum polarization,''
JHEP \textbf{08}, 137 (2019)
%doi:10.1007/JHEP08(2019)137
[arXiv:1907.01556 [hep-ph]].

\bibitem{Davier:2019can}
M.~Davier, A.~Hoecker, B.~Malaescu and Z.~Zhang,
%``A new evaluation of the hadronic vacuum polarisation contributions to the muon anomalous magnetic moment and to $\mathbf{\boldsymbol\alpha(m_Z^2)}$,''
Eur. Phys. J. C \textbf{80}, no.3, 241 (2020)
[erratum: Eur. Phys. J. C \textbf{80}, no.5, 410 (2020)]
%doi:10.1140/epjc/s10052-020-7792-2
[arXiv:1908.00921 [hep-ph]].

\bibitem{Keshavarzi:2019abf}
A.~Keshavarzi, D.~Nomura and T.~Teubner,
%``$g-2$ of charged leptons, $\alpha (M^2_Z)$ , and the hyperfine splitting of muonium,''
Phys. Rev. D \textbf{101}, no.1, 014029 (2020)
%doi:10.1103/PhysRevD.101.014029
[arXiv:1911.00367 [hep-ph]].

\bibitem{Kurz:2014wya}
A.~Kurz, T.~Liu, P.~Marquard and M.~Steinhauser,
%``Hadronic contribution to the muon anomalous magnetic moment to next-to-next-to-leading order,''
Phys. Lett. B \textbf{734}, 144-147 (2014)
%doi:10.1016/j.physletb.2014.05.043
[arXiv:1403.6400 [hep-ph]].

\bibitem{Melnikov:2003xd}
K.~Melnikov and A.~Vainshtein,
%``Hadronic light-by-light scattering contribution to the muon anomalous magnetic moment revisited,''
Phys. Rev. D \textbf{70}, 113006 (2004)
%doi:10.1103/PhysRevD.70.113006
[arXiv:hep-ph/0312226 [hep-ph]].

\bibitem{Masjuan:2017tvw}
P.~Masjuan and P.~Sanchez-Puertas,
%``Pseudoscalar-pole contribution to the $(g_{\mu}-2)$: a rational approach,''
Phys. Rev. D \textbf{95}, no.5, 054026 (2017)
%doi:10.1103/PhysRevD.95.054026
[arXiv:1701.05829 [hep-ph]].

\bibitem{Colangelo:2017fiz}
G.~Colangelo, M.~Hoferichter, M.~Procura and P.~Stoffer,
%``Dispersion relation for hadronic light-by-light scattering: two-pion contributions,''
JHEP \textbf{04}, 161 (2017)
%doi:10.1007/JHEP04(2017)161
[arXiv:1702.07347 [hep-ph]].

\bibitem{Hoferichter:2018kwz}
M.~Hoferichter, B.~L.~Hoid, B.~Kubis, S.~Leupold and S.~P.~Schneider,
%``Dispersion relation for hadronic light-by-light scattering: pion pole,''
JHEP \textbf{10}, 141 (2018)
%doi:10.1007/JHEP10(2018)141
[arXiv:1808.04823 [hep-ph]].

\bibitem{Gerardin:2019vio}
A.~G\'erardin, H.~B.~Meyer and A.~Nyffeler,
%``Lattice calculation of the pion transition form factor with $N_f=2+1$ Wilson quarks,''
Phys. Rev. D \textbf{100}, no.3, 034520 (2019)
%doi:10.1103/PhysRevD.100.034520
[arXiv:1903.09471 [hep-lat]].

\bibitem{Bijnens:2019ghy}
J.~Bijnens, N.~Hermansson-Truedsson and A.~Rodr\'\i{}guez-S\'anchez,
%``Short-distance constraints for the HLbL contribution to the muon anomalous magnetic moment,''
Phys. Lett. B \textbf{798}, 134994 (2019)
%doi:10.1016/j.physletb.2019.134994
[arXiv:1908.03331 [hep-ph]].

\bibitem{Colangelo:2019uex}
G.~Colangelo, F.~Hagelstein, M.~Hoferichter, L.~Laub and P.~Stoffer,
%``Longitudinal short-distance constraints for the hadronic light-by-light contribution to $(g-2)_\mu$ with large-$N_c$ Regge models,''
JHEP \textbf{03}, 101 (2020)
%doi:10.1007/JHEP03(2020)101
[arXiv:1910.13432 [hep-ph]].

\bibitem{Blum:2019ugy}
T.~Blum, N.~Christ, M.~Hayakawa, T.~Izubuchi, L.~Jin, C.~Jung and C.~Lehner,
%``Hadronic Light-by-Light Scattering Contribution to the Muon Anomalous Magnetic Moment from Lattice QCD,''
Phys. Rev. Lett. \textbf{124}, no.13, 132002 (2020)
%doi:10.1103/PhysRevLett.124.132002
[arXiv:1911.08123 [hep-lat]].

\bibitem{Colangelo:2014qya}
G.~Colangelo, M.~Hoferichter, A.~Nyffeler, M.~Passera and P.~Stoffer,
%``Remarks on higher-order hadronic corrections to the muon g\ensuremath{-}2,''
Phys. Lett. B \textbf{735}, 90-91 (2014)
%doi:10.1016/j.physletb.2014.06.012
[arXiv:1403.7512 [hep-ph]].
\bibitem{Pauk:2014rta}
V.~Pauk and M.~Vanderhaeghen,
%``Single meson contributions to the muon`s anomalous magnetic moment,''
Eur. Phys. J. C \textbf{74}, no.8, 3008 (2014)
%doi:10.1140/epjc/s10052-014-3008-y
[arXiv:1401.0832 [hep-ph]].

%%%%% 
\bibitem{Jegerlehner:2017gek}
F.~Jegerlehner,
%``The Anomalous Magnetic Moment of the Muon,''
Springer Tracts Mod. Phys. \textbf{274}, pp.1-693 (2017)
%doi:10.1007/978-3-319-63577-4

\bibitem{Knecht:2018sci}
M.~Knecht, S.~Narison, A.~Rabemananjara and D.~Rabetiarivony,
%``Scalar meson contributions to a \ensuremath{\mu} from hadronic light-by-light scattering,''
Phys. Lett. B \textbf{787}, 111-123 (2018)
%doi:10.1016/j.physletb.2018.10.048
[arXiv:1808.03848 [hep-ph]].

\bibitem{Eichmann:2019bqf}
G.~Eichmann, C.~S.~Fischer and R.~Williams,
%``Kaon-box contribution to the anomalous magnetic moment of the muon,''
Phys. Rev. D \textbf{101}, no.5, 054015 (2020)
%doi:10.1103/PhysRevD.101.054015
[arXiv:1910.06795 [hep-ph]].

\bibitem{Roig:2019reh}
P.~Roig and P.~Sanchez-Puertas,
%``Axial-vector exchange contribution to the hadronic light-by-light piece of the muon anomalous magnetic moment,''
Phys. Rev. D \textbf{101}, no.7, 074019 (2020)
%doi:10.1103/PhysRevD.101.074019
[arXiv:1910.02881 [hep-ph]].


%%%%%%%%%%%%%%%
\bibitem{Ghosh:2023dgk}
S.~Ghosh and P.~Ko,
%``Explaining ATOMKI, $(g-2)_\mu$, and MiniBooNE anomalies with light mediators in $U(1)_H$ extended model,''
[arXiv:2311.14099 [hep-ph]].





%%%%%(g-2)e
\bibitem{Hanneke:2008tm}
D.~Hanneke, S.~Fogwell and G.~Gabrielse,
%``New Measurement of the Electron Magnetic Moment and the Fine Structure Constant,''
Phys. Rev. Lett. \textbf{100} (2008), 120801
%doi:10.1103/PhysRevLett.100.120801
[arXiv:0801.1134 [physics.atom-ph]].



%\cite{Morel:2020dww}
\bibitem{Morel:2020dww}
L.~Morel, Z.~Yao, P.~Clad\'e and S.~Guellati-Kh\'elifa,
%``Determination of the fine-structure constant with an accuracy of 81 parts per trillion,''
Nature \textbf{588} (2020) no.7836, 61-65
%doi:10.1038/s41586-020-2964-7

\bibitem{Aoyama:2012wj}
T.~Aoyama, M.~Hayakawa, T.~Kinoshita and M.~Nio,
%``Tenth-Order QED Contribution to the Electron g-2 and an Improved Value of the Fine Structure Constant,''
Phys. Rev. Lett. \textbf{109} (2012), 111807
%doi:10.1103/PhysRevLett.109.111807
[arXiv:1205.5368 [hep-ph]].



\bibitem{Laporta:2017okg}
S.~Laporta,
%``High-precision calculation of the 4-loop contribution to the electron g-2 in QED,''
Phys. Lett. B \textbf{772} (2017), 232-238
%doi:10.1016/j.physletb.2017.06.056
[arXiv:1704.06996 [hep-ph]].

\bibitem{Aoyama:2017uqe}
T.~Aoyama, T.~Kinoshita and M.~Nio,
%``Revised and Improved Value of the QED Tenth-Order Electron Anomalous Magnetic Moment,''
Phys. Rev. D \textbf{97} (2018) no.3, 036001
%doi:10.1103/PhysRevD.97.036001
[arXiv:1712.06060 [hep-ph]].

\bibitem{Terazawa:2018pdc}
H.~Terazawa,
%``Convergence of Perturbative Expansion Series in QED and the Muon g-2: One of the Oldest Problems in Quantum Field Theory and of the Latest Problems in the Standard Model,''
Nonlin. Phenom. Complex Syst. \textbf{21} (2018) no.3, 268-272
%7 citations counted in INSPIRE as of 05 Feb 2023

\bibitem{Volkov:2019phy}
S.~Volkov,
%``Calculating the five-loop QED contribution to the electron anomalous magnetic moment: Graphs without lepton loops,''
Phys. Rev. D \textbf{100} (2019) no.9, 096004
%doi:10.1103/PhysRevD.100.096004
[arXiv:1909.08015 [hep-ph]].



\bibitem{Gerardin:2020gpp}
A.~G\'erardin,
%``The anomalous magnetic moment of the muon: status of Lattice QCD calculations,''
Eur. Phys. J. A \textbf{57} (2021) no.4, 116
%doi:10.1140/epja/s10050-021-00426-7
[arXiv:2012.03931 [hep-lat]].


\bibitem{BaBar:2009hkt}
B.~Aubert \textit{et al.} [BaBar],
%``Searches for Lepton Flavor Violation in the Decays tau+- ---\ensuremath{>} e+- gamma and tau+- ---\ensuremath{>} mu+- gamma,''
Phys. Rev. Lett. \textbf{104} (2010), 021802
%doi:10.1103/PhysRevLett.104.021802
[arXiv:0908.2381 [hep-ex]].

\bibitem{MEG:2016leq}
A.~M.~Baldini \textit{et al.} [MEG],
%``Search for the lepton flavour violating decay $\mu ^+ \rightarrow \mathrm {e}^+ \gamma $ with the full dataset of the MEG experiment,''
Eur. Phys. J. C \textbf{76} (2016) no.8, 434
%doi:10.1140/epjc/s10052-016-4271-x
[arXiv:1605.05081 [hep-ex]].

\bibitem{Belle:2021ysv}
A.~Abdesselam \textit{et al.} [Belle],
%``Search for lepton-flavor-violating tau-lepton decays to $\ell\gamma$ at Belle,''
JHEP \textbf{10} (2021), 19
%doi:10.1007/JHEP10(2021)019
[arXiv:2103.12994 [hep-ex]].

\bibitem{MEGII:2018kmf}
A.~M.~Baldini \textit{et al.} [MEG II],
%``The design of the MEG II experiment,''
Eur. Phys. J. C \textbf{78} (2018) no.5, 380
%doi:10.1140/epjc/s10052-018-5845-6
[arXiv:1801.04688 [physics.ins-det]].

\bibitem{Belle-II:2018jsg}
E.~Kou \textit{et al.} [Belle-II],
%``The Belle II Physics Book,''
PTEP \textbf{2019} (2019) no.12, 123C01
[erratum: PTEP \textbf{2020} (2020) no.2, 029201]
%doi:10.1093/ptep/ptz106
[arXiv:1808.10567 [hep-ex]].

%
\bibitem{CMS:2021rsq}
A.~M.~Sirunyan \textit{et al.} [CMS],
%``Search for lepton-flavor violating decays of the Higgs boson in the $\mu\tau$ and e$\tau$ final states in proton-proton collisions at $\sqrt{s}$ = 13 TeV,''
Phys. Rev. D \textbf{104} (2021) no.3, 032013 
%doi:10.1103/PhysRevD.104.032013
[arXiv:2105.03007 [hep-ex]].

\bibitem{ATLAS:2019xlq}
[ATLAS],
``Search for the decays of the Higgs boson $H \to ee$ and $H \to e\mu$ in $pp$ collisions at $\sqrt{s}$ = 13 TeV with the ATLAS detector,''
ATLAS-CONF-2019-037


\bibitem{Qin:2017aju}
Q.~Qin, Q.~Li, C.~D.~L\"u, F.~S.~Yu and S.~H.~Zhou,
%``Charged lepton flavor violating Higgs decays at future $e^+e^-$ colliders,''
Eur. Phys. J. C \textbf{78} (2018) no.10, 835
%doi:10.1140/epjc/s10052-018-6298-7
[arXiv:1711.07243 [hep-ph]].

\bibitem{Barman:2022iwj}
R.~K.~Barman, P.~S.~B.~Dev and A.~Thapa,
%``Constraining lepton flavor violating Higgs couplings at the HL-LHC in the vector boson fusion channel,''
Phys. Rev. D \textbf{107} (2023) no.7, 075018
%doi:10.1103/PhysRevD.107.075018
[arXiv:2210.16287 [hep-ph]].

\bibitem{Aoki:2023wfb}
M.~Aoki, S.~Kanemura, M.~Takeuchi and L.~Zamakhsyari,
%``Probing the chirality structure in the lepton-flavor-violating Higgs decay h\textrightarrow{}\ensuremath{\tau}\ensuremath{\mu} at the LHC,''
Phys. Rev. D \textbf{107} (2023) no.5, 055037
%doi:10.1103/PhysRevD.107.055037
[arXiv:2302.08489 [hep-ph]].

\bibitem{ATLAS:2021bdj}
G.~Aad \textit{et al.} [ATLAS],
%``Search for lepton-flavor-violation in $Z$-boson decays with $\tau$-leptons with the ATLAS detector,''
Phys. Rev. Lett. \textbf{127} (2022), 271801
%doi:10.1103/PhysRevLett.127.271801
[arXiv:2105.12491 [hep-ex]].

\bibitem{ATLAS:2022uhq}
G.~Aad \textit{et al.} [ATLAS],
%``Search for the charged-lepton-flavor-violating decay $Z\rightarrow e\mu$ in $pp$ collisions at $\sqrt{s}=13$ TeV with the ATLAS detector,''
Phys. Rev. D \textbf{108} (2023), 032015
%doi:10.1103/PhysRevD.108.032015
[arXiv:2204.10783 [hep-ex]].

\bibitem{Dam:2018rfz}
M.~Dam,
%``Tau-lepton Physics at the FCC-ee circular e$^+$e$^-$ Collider,''
SciPost Phys. Proc. \textbf{1} (2019), 041
%doi:10.21468/SciPostPhysProc.1.041
[arXiv:1811.09408 [hep-ex]].

\bibitem{FCC:2018byv}
A.~Abada \textit{et al.} [FCC],
%``FCC Physics Opportunities: Future Circular Collider Conceptual Design Report Volume 1,''
Eur. Phys. J. C \textbf{79} (2019) no.6, 474
%doi:10.1140/epjc/s10052-019-6904-3


\bibitem{Grimus:2002ux}
W.~Grimus and L.~Lavoura,
%``Soft lepton flavor violation in a multi Higgs doublet seesaw model,''
Phys. Rev. D \textbf{66} (2002), 014016
%doi:10.1103/PhysRevD.66.014016
[arXiv:hep-ph/0204070 [hep-ph]].

\bibitem{Dreiner:2008tw}
H.~K.~Dreiner, H.~E.~Haber and S.~P.~Martin,
%``Two-component spinor techniques and Feynman rules for quantum field theory and supersymmetry,''
Phys. Rept. \textbf{494} (2010), 1-196
%doi:10.1016/j.physrep.2010.05.002
[arXiv:0812.1594 [hep-ph]].

\bibitem{Branco:2011iw}
G.~C.~Branco, P.~M.~Ferreira, L.~Lavoura, M.~N.~Rebelo, M.~Sher and J.~P.~Silva,
%``Theory and phenomenology of two-Higgs-doublet models,''
Phys. Rept. \textbf{516} (2012), 1-102
%doi:10.1016/j.physrep.2012.02.002
[arXiv:1106.0034 [hep-ph]].


\bibitem{tHooft:1978jhc}
G.~'t Hooft and M.~J.~G.~Veltman,
%``Scalar One Loop Integrals,''
Nucl. Phys. B \textbf{153} (1979), 365-401
%doi:10.1016/0550-3213(79)90605-9

\bibitem{Vermaseren:2000nd}
J.~A.~M.~Vermaseren,
%``New features of FORM,''
[arXiv:math-ph/0010025 [math-ph]].

\bibitem{Kuipers:2012rf}
J.~Kuipers, T.~Ueda, J.~A.~M.~Vermaseren and J.~Vollinga,
%``FORM version 4.0,''
Comput. Phys. Commun. \textbf{184} (2013), 1453-1467
%doi:10.1016/j.cpc.2012.12.028
[arXiv:1203.6543 [cs.SC]].


\bibitem{Casas:2001sr}
J.~A.~Casas and A.~Ibarra,
%``Oscillating neutrinos and $\mu \to e, \gamma$,''
Nucl. Phys. B \textbf{618} (2001), 171-204
%doi:10.1016/S0550-3213(01)00475-8
[arXiv:hep-ph/0103065 [hep-ph]].

\bibitem{ParticleDataGroup:2022pth}
R.~L.~Workman \textit{et al.} [Particle Data Group],
%``Review of Particle Physics,''
PTEP \textbf{2022} (2022), 083C01
%doi:10.1093/ptep/ptac097

\bibitem{Thao:2017qtn}
N.~H.~Thao, L.~T.~Hue, H.~T.~Hung and N.~T.~Xuan,
%``Lepton flavor violating Higgs boson decays in seesaw models: new discussions,''
Nucl. Phys. B \textbf{921} (2017), 159-180
%doi:10.1016/j.nuclphysb.2017.05.014
[arXiv:1703.00896 [hep-ph]].

\bibitem{Hue:2021zyw}
L.~T.~Hue, K.~H.~Phan, T.~P.~Nguyen, H.~N.~Long and H.~T.~Hung,
%``An explanation of experimental data of $(g-2)_{e,\mu }$ in 3-3-1 models with inverse seesaw neutrinos,''
Eur. Phys. J. C \textbf{82} (2022) no.8, 722
%doi:10.1140/epjc/s10052-022-10691-5
[arXiv:2109.06089 [hep-ph]].


\bibitem{Pilaftsis:1992st}
A.~Pilaftsis,
%``Lepton flavor nonconservation in H0 decays,''
Phys. Lett. B \textbf{285} (1992), 68-74
%doi:10.1016/0370-2693(92)91301-O

\bibitem{Arganda:2004bz}
E.~Arganda, A.~M.~Curiel, M.~J.~Herrero and D.~Temes,
%``Lepton flavor violating Higgs boson decays from massive seesaw neutrinos,''
Phys. Rev. D \textbf{71} (2005), 035011
%doi:10.1103/PhysRevD.71.035011
[arXiv:hep-ph/0407302 [hep-ph]].

\bibitem{LHCHiggsCrossSectionWorkingGroup:2016ypw}
D.~de Florian \textit{et al.} [LHC Higgs Cross Section Working Group],
%``Handbook of LHC Higgs Cross Sections: 4. Deciphering the Nature of the Higgs Sector,''
%doi:10.23731/CYRM-2017-002
[arXiv:1610.07922 [hep-ph]].


\bibitem{Lavoura:2003xp}
L.~Lavoura,
%``General formulae for f(1) ---\ensuremath{>} f(2) gamma,''
Eur. Phys. J. C \textbf{29}, 191-195 (2003)
%doi:10.1140/epjc/s2003-01212-7
[arXiv:hep-ph/0302221 [hep-ph]].


\bibitem{Hue:2017lak}
L.~T.~Hue, L.~D.~Ninh, T.~T.~Thuc and N.~T.~T.~Dat,
%``Exact one-loop results for $l_i \to l_j\gamma$ in 3-3-1 models,''
Eur. Phys. J. C \textbf{78} (2018) no.2, 128
%doi:10.1140/epjc/s10052-018-5589-3
[arXiv:1708.09723 [hep-ph]].

\bibitem{Hue:2021xzl}
L.~T.~Hue, A.~E.~C\'arcamo Hern\'andez, H.~N.~Long and T.~T.~Hong,
%``Heavy singly charged Higgs bosons and inverse seesaw neutrinos as origins of large (g\ensuremath{-}2)e,\ensuremath{\mu} in two Higgs doublet models,''
Nucl. Phys. B \textbf{984} (2022), 115962
%doi:10.1016/j.nuclphysb.2022.115962
[arXiv:2110.01356 [hep-ph]].

\bibitem{Planck:2018vyg}
N.~Aghanim \textit{et al.} [Planck],
%``Planck 2018 results. VI. Cosmological parameters,''
Astron. Astrophys. \textbf{641} (2020), A6
[erratum: Astron. Astrophys. \textbf{652} (2021), C4]
%doi:10.1051/0004-6361/201833910
[arXiv:1807.06209 [astro-ph.CO]].

\bibitem{Agostinho:2017wfs}
N.~R.~Agostinho, G.~C.~Branco, P.~M.~F.~Pereira, M.~N.~Rebelo and J.~I.~Silva-Marcos,
%``Can one have significant deviations from leptonic 3 $\times $ 3 unitarity in the framework of type I seesaw mechanism?,''
Eur. Phys. J. C \textbf{78} (2018) no.11, 895
%doi:10.1140/epjc/s10052-018-6347-2
[arXiv:1711.06229 [hep-ph]].


\bibitem{Coutinho:2019aiy}
A.~M.~Coutinho, A.~Crivellin and C.~A.~Manzari,
%``Global Fit to Modified Neutrino Couplings and the Cabibbo-Angle Anomaly,''
Phys. Rev. Lett. \textbf{125} (2020) no.7, 071802
%doi:10.1103/PhysRevLett.125.071802
[arXiv:1912.08823 [hep-ph]].

\bibitem{Biggio:2019eeo}
C.~Biggio, E.~Fernandez-Martinez, M.~Filaci, J.~Hernandez-Garcia and J.~Lopez-Pavon,
%``Global Bounds on the Type-III Seesaw,''
JHEP \textbf{05} (2020), 022
%doi:10.1007/JHEP05(2020)022
[arXiv:1911.11790 [hep-ph]].

\bibitem{Escribano:2021css}
P.~Escribano, J.~Terol-Calvo and A.~Vicente,
%``$\boldsymbol{(g-2)_{e,\mu}}$ in an extended inverse type-III seesaw model,''
Phys. Rev. D \textbf{103} (2021) no.11, 115018
%doi:10.1103/PhysRevD.103.115018
[arXiv:2104.03705 [hep-ph]].

\bibitem{Thao:2023gvs}
N.~H.~Thao, D.~T.~Binh, T.~T.~Hong, L.~T.~Hue and D.~P.~Khoi,
%``$(g-2)_{e,\mu}$ and decays $e_b\to e_a\gamma$ in a $ \mbox{SU}(4)_L \otimes \mbox{U}(1)_X$ model with inverse seesaw neutrinos,''
PTEP \textbf{2023} (2023), 8
%doi:10.1093/ptep/ptad092
[arXiv:2302.07576 [hep-ph]].

\bibitem{tHooft:1972tcz}
G.~'t Hooft and M.~J.~G.~Veltman,
%``Regularization and Renormalization of Gauge Fields,''
Nucl. Phys. B \textbf{44} (1972), 189-213
%doi:10.1016/0550-3213(72)90279-9


\bibitem{Hahn:1998yk}
T.~Hahn and M.~Perez-Victoria,
%``Automatized one loop calculations in four-dimensions and D-dimensions,''
Comput. Phys. Commun. \textbf{118} (1999), 153-165
%doi:10.1016/S0010-4655(98)00173-8
[arXiv:hep-ph/9807565 [hep-ph]].


\bibitem{Peskin:1995ev}
M.~E.~Peskin and D.~V.~Schroeder,
%``An Introduction to quantum field theory,''
Addison-Wesley, 1995,
ISBN 978-0-201-50397-5

\bibitem{Nguyen:2020ehj}
T.~P.~Nguyen, T.~T.~Thuc, D.~T.~Si, T.~T.~Hong and L.~T.~Hue,
%``Low-energy phenomena of the lepton sector in an A4 symmetry model with heavy inverse seesaw neutrinos,''
PTEP \textbf{2022} (2022) no.2, 023B01
%doi:10.1093/ptep/ptac002
[arXiv:2011.12181 [hep-ph]].


\bibitem{Nguyen:2018rlb}
T.~P.~Nguyen, T.~T.~Le, T.~T.~Hong and L.~T.~Hue,
%``Decay of standard model-like Higgs boson $h\rightarrow \mu\tau$ in a 3-3-1 model with inverse seesaw neutrino masses,''
Phys. Rev. D \textbf{97} (2018) no.7, 073003
%doi:10.1103/PhysRevD.97.073003
[arXiv:1802.00429 [hep-ph]].




\bibitem{Hue:2015fbb}
L.~T.~Hue, H.~N.~Long, T.~T.~Thuc and T.~Phong Nguyen,
%``Lepton flavor violating decays of Standard-Model-like Higgs in 3-3-1 model with neutral lepton,''
Nucl. Phys. B \textbf{907} (2016), 37-76
%doi:10.1016/j.nuclphysb.2016.03.034
[arXiv:1512.03266 [hep-ph]].

\crb{
\bibitem{Cherchiglia:2023utd}
A.~L.~Cherchiglia, G.~De Conto and C.~C.~Nishi,
%``Connecting (g \ensuremath{-} 2)$_{μ}$ to neutrino mass in the extended neutrinophilic 2HDM,''
JHEP \textbf{08} (2023), 170
%doi:10.1007/JHEP08(2023)170
[arXiv:2304.00038 [hep-ph]].
}




%%%%%%%%%%%%%%%%%orderref%%%%%%





















































